IsoPredict: Dynamic Predictive Analysis for Detecting Unserializable Behaviors in Weakly Isolated Data Store Applications

This paper presents the first dynamic predictive analysis for data store applications under weak isolation levels, called Isopredict. Given an observed serializable execution of a data store application, Isopredict generates and solves SMT constraints to find an unserializable execution that is a feasible execution of the application. Isopredict introduces novel techniques that handle divergent application behavior; solve mutually recursive sets of constraints; and balance coverage, precision, and performance. An evaluation on four transactional data store benchmarks shows that Isopredict often predicts unserializable behaviors, 99% of which are feasible.

==> cover.tex <==
\UseRawInputEncoding

\noindent
Dear Reviewers,

~

\noindent
% We would like to
Thank you for the thoughtful reviews of our work. This document describes revisions in response to reviewer feedback from the last round, followed by the revised paper for convenience.
% including the appendix with supplementary material.

\section*{Revisions}

\begin{empty}
\lstset{%
  language=[LaTeX]TeX,
  backgroundcolor=\color{gray!25},
  basicstyle=\ttfamily\small,
  breaklines=true,
  columns=fullflexible,
  comment=[l]{},
  %breakautoindent=false,
  %autoindent=false,
  breakindent=0pt,
  breakatwhitespace=true,
  keepspaces=true,
  %literate={-}{-}1
  literate    ={–}{\textendash}1 {—}{\textemdash}2,
  escapeinside={(*@}{@*)},
}

We have revised the paper to respond to all reviewer feedback.
Details of how we responded to each comment are inlined into the reviews below, starting with the required revisions from the meta review.
\iffalse
Highlights:
\begin{itemize}
\item TODO
\item TODO
\item TODO
\end{itemize}
In the following, we mostly point to our paper revisions rather than providing a response here.
\fi

\newcommand{\response}[1]{\noindent\textcolor{ACMDarkBlue}{#1}}
% \newcommand{\response}[1]{\noindent \textcolor{darkgray}{#1}}

\begin{lstlisting}
Review #59E
===========================================================================

Overall merit
-------------
5. Strong accept

Reviewer expertise
------------------
1. No familiarity

Paper summary
-------------
This is the meta review.

Comments for authors
--------------------
Dear PLDI Authors of Paper #59 –

Congratulations! Your paper has been conditionally accepted by the 2024 PLDI Program Committee. Below, we detail the required and optional revisions we would like to see in the final draft of your paper for full acceptance.

While the reviewers are excited and positive about the impact of your paper, there are three areas where we would like to see improvements in your paper. They are as follows:

1.	[ Required ] Present a more detailed comparison against the body of related work cited in the reviews (especially those found in Review A and D).
\end{lstlisting}

\response{Improved and expanded the comparison with 2AD~\cite{Warszawski2017ACIDRain}, IsoDiff~\cite{isodiff}, and Sinha et al.'s analysis~\cite{sinha2012} in \S\ref{sec:related}. Added mention of other axiomatic encodings of weak isolation levels in \S\ref{sec:related}.}

\begin{lstlisting}
2.	[ Required ] Provide a deeper discussion on the challenges (if any) of your approach to support richer levels of isolation. (This is optional if you believe there are no specific challenges for your approach with other forms of isolation.)
\end{lstlisting}

\response{Revised (but did not substantially deepen) discussion of other isolation levels in \S\ref{sec:related}.}

\begin{lstlisting}
3.	[ Required ] Comment more substantively and empirically on an analysis of the long constraint solving times. We would prefer to have concrete data explain what is happening here rather than a potential mischaracterization of a PL's runtime causing (or not causing) the overhead.
\end{lstlisting}

\response{We investigated the long constraint generation times by measuring the size of the generated constraints and by running performance analysis on constraint generation. Tables~\ref{tab:oltpinfo}, \ref{tab:results_full_causal}, and \ref{tab:results_full_rc} now report the sizes (number of literals) of the generated constraints, which correlate with constraint generation times. Using a performance profiler, we found that a large fraction of constraint generation time is spent inside Z3Py, as Section~\ref{subsec:isopredict-results} now describes. (We report the fraction of time for only a single run of constraint generation because we had to manually compute the fraction from a flame graph.)}

\begin{lstlisting}
Justin Gottschlich will act as your paper shepherd. He can be reached at justin@merly.ai or goju@stanford.edu.

Thank you and we look forward to seeing a revision of your paper in the coming weeks.

Best,
2024 PLDI Program Committee

Review #59A
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
4. Expert

Paper summary
-------------
This paper considers the problem of determining a feasible
unserializable execution from a feasible serializable execution trace.
The basic idea is to encode various data dependencies induced by
program (write-read, write-write, read-write), session, and commit
ordering constraints, along with constraints required to enforce a
particular isolation level (causal or read-committed are the two
considered in the paper), and then asking a theorem prover whether
there exists a valid execution consistent with these constraints that
is unserializable (i.e., an execution that admits a cyclic dependence
among committed transactions).  Deriving new predicted executions may
lead to different behaviors (i.e., reads may return different values
by reading from a different transaction than in the original trace).
IsoPredict accounts for divergent executions (predicted executions
that are not validated) by potentially excluding events that lead to
such executions from consideration, raising the possibility that a
claimed unserializable execution is in fact serializable.  A
validation phase is thus available to check that candidate predictions
are correct.

Comments for authors
--------------------
Pros:
------

- Assessing the robustness of distributed data store applications against
weak isolation levels is an important and topical problem.

- The presented approach provides a principled, constraint-based,
solution to the problem.

- The solution to dealing with divergent behavior offers interesting
precision tradeoffs of the predictor.

Cons:
------

- The paper's novelty over prior work is modest given that the notion
of developing axiomatic encodings of weak isolation behavior has been
well-explored (e.g, 11, 34, Cerone et al (CONCUR'15), Kaki et
al. (OOPSLA'18)).  The 2AD analysis given in [44] leverages a similar
setup to IsoPredict, and is also a dynamic predictive analysis for
weak isolation.
\end{lstlisting}

\response{Addressed as part of required revisions.}

\begin{lstlisting}
- The paper only considers CC and RC; other important
isolation levels (MAV, RR, SI, PSI, etc.) are not discussed.
\end{lstlisting}

\response{Addressed as part of required revisions.}

\begin{lstlisting}
- Constraint generation times can be large (approaching 10 minutes
for some of the TPC-C variants).  Proving that there are no
unserializable behaviors using the same setup for generating a
counterexample doesn't seem to be practical.

- The evaluation is limited, conducted using a small number of
sessions (3) and transactions (12).  There is little discussion on the
scalability of the approach to longer executions.  As a related point,
many of the considered benchmarks have been previously successfully
investigated using static techniques.
\end{lstlisting}

\response{We're planning to incorporate Appendix~\ref{sec:scalability-results}'s results into the main paper for the camera-ready version.
\medskip\\
In any case, we'll include remaining appendices in an extended arXiv version of the paper.}

\begin{lstlisting}
- The approach only tracks fidelity against serializability, and
does not consider the integrity of application-specified invariants
under different isolation levels.

Comments:
------------

Although the problem considered by the paper is an interesting one,
it's also a topic that has been fairly well-explored.  MonkeyDB, as
the paper concedes, is closely related in terms of mechanism and
formulation, and 2AD ([44]) also presents a dynamic analysis for weak
isolation that searches for cycles in abstract histories, a compact
representation of an execution trace.  In this regard, I would have liked
to have seen more details on the benefits of the approach taken by IsoPredict
as compared to 2AD, i.e., why is the constraint generation and solving strategy
adopted in this paper a better formulation of a solution than the cycle detection
procedure used in 2AD, especially since both approaches can report false
positives, claiming a predicted execution to be unserializable even
when it is, and thus require a separate validation phase.
\end{lstlisting}

\response{Addressed as part of required revisions.}

\begin{lstlisting}
While the consideration of divergent computation is a novel
contribution, as far as I can tell, the distinction between the
strict and relaxed variants in terms of constraint generation and
solving times seem negligble in general.  Using a "relaxed"
prediction boundary seems to modestly improve identifying
unserializable executions for CC, while exhibiting no difference on
RC.  There's not much discussion in the paper for why these differences
(or lack thereof) manifest the way they do.

I view the results comparing IsoPredict with MonkeyDB to be mostly
inconclusive, with each demonstrating advantages over the other
on different benchmarks, but agree with the authors that the two systems
are intended to operate in different settings.

As the authors concede, the existing (non-optimized) implementation
results in long constraint generation times that weakens the claim on
the benefit of dynamic analysis in this setting over a static
approach.  In the absence of a more detailed scalability study, it's
unlikely IsoPredict as currently implemented can be used to analyze
realistic workloads.

The paper only considers two isolation levels (CC and RC), but does
not provide any intuition for why the results derived for these would
generalize to others (e.g., snapshot isolation, repeatable read, etc.)
\end{lstlisting}

\response{Addressed as part of required revisions.}

\begin{lstlisting}
Review #59B
===========================================================================

Overall merit
-------------
4. Accept

Reviewer expertise
------------------
4. Expert

Paper summary
-------------
The paper is concerned with the problem of checking correctness for distributed applications running on top of weakly-consistent transactional databases. It presents a procedure that takes as input a serializable execution and synthesizes other executions that are not serializable but consistent with a given weaker isolation level. The synthesis procedure is based on encoding consistency constraints in SMT based on the axiomatic theory introduced by Biswas et al. 2019. The synthesized executions are also validated by re-running the application since in principle, they may not be anymore admitted (reading different values may disable some of the events from the input serializable execution). The approach is implemented by running applications on top of MonkeyDB [Biswas et al. 2021], and evaluated on a number of applications from OLTP-Bench including TPCC.

Comments for authors
--------------------
Strengths:

Applications running on top of weak consistency are difficult to reason about.

The formalization is clear and well presented.

An approximate encoding of non-serializability to SMT which offers more performance while being precise enough in practice.

The evaluation is quite thorough. 

Weaknesses: 

The overall approach is quite standard. 

Comments:

In general, I think that this is a well-executed paper. It deals with an important and timely problem, it offers a solution which is effective while being incomparable to previous work, and the implementation is evaluated on realistic use-cases. While following the rather classic path of predictive analysis, it considers the specificities of the domain and in particular, it provides an approximate encoding of strong consistency to SMT (Section 4.2.2) which I found novel and quite interesting. As a side comment, could you give an example which shows why this encoding is approximate, a history for which this formula is unsat but which admits an unserializable prediction ?
\end{lstlisting}

\response{We still haven't been able to come up with an example. Added discussion at the end of Section~\ref{subsubsec:sufficient-unser-constraints}.}

\begin{lstlisting}
I am slightly confused about the validation phase. If I understand correctly, you are using the fact that MonkeyDB makes it possible to control the transaction that some read is reading from. I wonder how the validation would be done on a regular database used as a blackbox. One option is running an application many times hoping to observe the predicted execution. But then, witnessing weak behaviors using standard setups of databases is rather difficult. Can you clarify the dependency of the validation phase on MonkeyDB ?
\end{lstlisting}

\response{Added discussion paragraph in Section~\ref{subsubsec:validating-execution}.}

\begin{lstlisting}
Review #59C
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
3. Knowledgeable

Paper summary
-------------
This submission proposes an SMT-based approach to predict unserializable executions of a distributed data stores from their serializable executions. The authors present IsoPredict, which translates observed (serializable) executions into SMT constraints whose satisfying assignments predict potential unserializable executions, which are then validated against a given data store. To reduce the constraint-solving burden, the authors also propose weaker approximating constraints. While the weaker constraints can, in principle, predict executions which are actually serializable, in practice, these weaker constraints do not produce spurious predictions, and are more efficiently solvable. Furthermore, to mitigate the effects of divergence between the events of the observed and predicted executions, the authors introduce a notion of "boundaries" into their constraints which are used to exclude subsequent events (strict variant) or transitions (relaxed variant) following events which read from distinct transitions from the observed to predicted execution. Empirically, the authors demonstrate the efficacy of their approach on transactional workloads from a relational-database benchmark set.

Comments for authors
--------------------
### Strengths

* IsoPredict's approximate constraints yield significant performance improvement with seemingly-negligible false positive rate.
* IsoPredict can account for (non-abort related) divergences between observed and predicted executions.
* Empirically IsoPredict appears to be very effective in predicting unserializable executions.

### Weaknesses

* While the authors note that "transactional applications on data stores present unique challenges compared with shared-memory programs" when comparing to predictive analysis for shared-memory programs, the technical novelty of IsoPredict, compared to existing approaches to predictive analysis shared-memory programs, is not obviously significant. While it is clear that Sinha et al.'s work, for instance, would differ in the precise formulation of SMT constraints, since they presumably deal with different consistency models, it is unclear whether those differences follow directly from the differing definitions of happens-before for the underlying consistency model. In other words, can we justify novelty simply in IsoPredict's formulations of causal and RC?
\end{lstlisting}

\response{Addressed as part of required revisions.}

\begin{lstlisting}
* Similarly, it is not clear to what extent the other aspects of IsoPredict aside from prediction-constraint satisfiability problem, e.g., validation, are novel.

* The authors point out that others "[do] not have to deal with divergence due to transaction aborts", but it appears that IsoPredict also does not — the provided "boundary" functions seem to deal only with divergence that are not caused by aborts.
\end{lstlisting}

\response{That's a valid point: \Isopredict only ``deals with'' divergence in the sense that it needs validation to be 100\% precise even when using the strict prediction boundary. Removed that sentence from Section~\ref{sec:related}.}

\begin{lstlisting}
* While the empirical validation seems very positive, I'm not quite sure how to interpret the results, nor to what extent the provided benchmark set is provides substantial confidence in the results. For example, is it surprising that the studied applications admit unserializable executions, or are such executions easy to observe in practice? (In the latter case, why bother with this expensive prediction mechanism at all?)
\end{lstlisting}

\response{We ran the benchmarks on MySQL and reported the results in Table~\ref{subtab:comparison-rc-small} and Section~\ref{subsec:cmp_monkeydb}.}

\begin{lstlisting}
Review #59D
===========================================================================

Overall merit
-------------
4. Accept

Reviewer expertise
------------------
4. Expert

Paper summary
-------------
This paper presents IsoPredict, a novel system to detect unserializable, yet observable executions. Unserializability is the notion that a program schedule (or execution) cannot be represented as a serial ordering of events. In this particular case, the "events" that the authors are referring to in a serial order are transactions (but in other contexts it could also refer to mutexes, atomic regions, etc.).

The authors demonstrate the efficacy of their system on four data store benchmarks and show that 99% of the unserializable schedules are observable (i.e., feasible, possible). Moreover, they demonstrate the technical differentiation of their approach compared to other state-of-the-art systems, such as MonkeyDB. A core difference between MonkeyDB and IsoPredict is that IsoPredict doesn't find unserialable schedules in a brute force fashion, as is done with MonkeyDB. Instead, IsoPredict uses predictive analysis to find them.

Comments for authors
--------------------
Note: I did not have time to precisely verify all of the formal theory used in the paper. However, I did review all of the theoretical contributions. There was nothing in it that jumped out as incorrect to me. That said, it is possible I've missed something.

Strengths:

+ The paper is masterfully written, including nearly perfectly written prose to precisely explain the formal mathematics used in the paper
+ The paper targets the important open problem of weak isolation, which is commonly used in many databases to promote scalability even though it is possible to incur correctness issues (or stale views)
+ The authors demonstrate mastery over the subject matter and clearly articulate the current state of things as well as the challenges inherent in them (e.g., why weak isolation is used, but why it can be problematic, especially if it results in unserializable schedules)
+ Both the formal theory and experimental results are sound

Weaknesses:

- Due to the complexity of the topic, it's likely that a novice reader may have some trouble with the topic. I'm not sure this is really a weakness of the paper, but more a point that the topic is complex and the authors approach it with an equally sophisticated solution.
- Did the experimental machine really have 191GB of RAM? :) That seems like a strange number. Are you sure it wasn't 192GB?
\end{lstlisting}

\response{It turns out the machine actually has 187\,GB, confirmed via both \texttt{/proc/meminfo} and \texttt{lstopo}. (We mistakenly reported 191\,GB because 187\,GB $\approx$ 191,000\,MB.)}

\begin{lstlisting}
- Try as I might, I can't find much wrong with this paper ... which is unusual for me.
\end{lstlisting}

\end{empty}


==> monkeydb_bugs.tex <==
\section{Bugs in MonkeyDB}
\label{sec:monkeydb_bugs}

\mike{Mention in Impl that we'll make everything publicly available.}

We found the following bugs in MonkeyDB (version: 6bff20e). The authors from MonkeyDB confirmed both our findings and our fixes.

\paragraph{Typo in the \bench{Smallbank} program of the ported OLTP Benchmark}
The typo was on line 9 of Listing~\ref{lst:bug_smallbank} where $\mathit{updateStmt0}$ should have been replaced with $\mathit{updateStmt1}$.
Otherwise, $\mathit{custId0}$'s checking balance would be updated to zero while the saving balance remained unchanged, resulting in an unexpected ending balance.
After fixing the typo, the assertion violation rate in \bench{Smallbank} decreased from 80\% to 70\% under causal consistency.

\begin{Java}[caption={Typo in Amalgamate.java}, label={lst:bug_smallbank}]
public void run(Connection conn, long custId0, long custId1) throws SQLException {
...
PreparedStatement updateStmt0 = this.getPreparedStatement(conn, ZeroCheckingBalance, custId0);
int status = updateStmt0.executeUpdate();
assert(status == 1);

PreparedStatement updateStmt1 = this.getPreparedStatement(conn, ZeroSavingsBalance, custId0);
status = updateStmt0.executeUpdate();
assert(status == 1);

PreparedStatement updateStmt2 = this.getPreparedStatement(conn, UpdateCheckingBalance, total, custId1);
status = updateStmt2.executeUpdate();
assert(status == 1);
...
}
\end{Java}

\paragraph{Initial values of \bench{Wikipeida}'s edit counts do not match MonkeyDB's assertions}
The assertions for \bench{Wikipedia} check whether all user's page edit records match those from the $\mathit{recentchanges}$ table (Listing~\ref{lst:bug_wiki_1}) and the $\mathit{logging}$ table.
However, the assertions wrongfully assume the initial value of every user's $\mathit{usereditcount}$ is zero, which is in fact a hard-coded non-zero value.
We fixed this bug by hard-coding zeroes for all user's initial $\mathit{usereditcount}$.
\begin{Rust}[caption={An assertion for \bench{Wikipedia} that checks if users' edits are consistent with the records from $\mathit{recentchanges}$ table.}, label={lst:bug_wiki_1}]
fn cr01(conn: &mut Conn) -> bool {
    // Total number of changes done for all the pages by each user in recentchanges = no.of pages
    // edited by individual user useracct

    // SELECT user_id, user_editcount FROM useracct
    // SELECT rc_user, count(*) FROM recentchanges GROUP BY rc_user

    /*
    SELECT * FROM
    (SELECT user_id, user_editcount FROM useracct)
    JOIN
    (SELECT rc_user, count(*) as rc_count FROM recentchanges GROUP BY rc_user)
    ON (user_id = rc_user)
    WHERE user_editcount != rc_count;
    */

    let mut change_cnt = HashMap::new();

    let result = conn
        .query_iter("SELECT user_id, user_editcount FROM useracct")
        .unwrap();

    for mut row in result.flatten() {
        let user_id: u64 = row.take::<String, _>("user_id").unwrap().parse().unwrap();
        let user_editcount: u64 = row
            .take::<String, _>("user_editcount")
            .unwrap()
            .parse()
            .unwrap();

        change_cnt.insert(user_id, user_editcount);
    }

    let result = conn
        .query_iter("SELECT rc_user FROM recentchanges")
        .unwrap();

    for mut row in result.flatten() {
        let rc_user: u64 = row.take::<String, _>("rc_user").unwrap().parse().unwrap();

        let ent = change_cnt.entry(rc_user).or_default();
        *ent -= 1;
    }

    change_cnt.values().all(|x| x == &0)
}
\end{Rust}

\paragraph{MonkeyDB's assertion checking module for \bench{Wikipedia} did not consider anonymous users' corner case}
The second bug fix in \bench{Wikipeida} is about anonymous user's updates. 
These updates are recorded in the $\mathit{recentchanges}$ table and the $\mathit{logging}$ table, but they don't show up in the $\mathit{users}$ table. 
The assertions treated them like normal users and were likely to end up with a mismatched $\mathit{usereditcount}$ number when there are updates from the anonymous users. 
We fixed the bug by ignoring anonymous users' edits in the assertion checks.
After the fixes to \bench{Wikipedia}'s assertions, MonkeyDB's assertion violation rate dropped to near 0 under \causal, which probably indicates that these assertions provide a lower coverage under \causal as compared to assertions for other benchmark programs.

==> results/benchmarks.tex <==
\newcommand\mytx[2]{#2 & (#1)}

% \begin{subtable}[t]{\textwidth}
\centering
\begin{tabular}{l|rr|rr}
& \mc{2}{c|}{\bf KV accesses} & \mc{2}{c}{\bf Committed txns} \\
\bf Program & Reads & Writes & Total & (Read-only)  \\
\hline
\bench{Smallbank} & 669.7 & 14.7 & \mytx{3.5}{11.0} \\
\bench{Voter} & 763.0 & 6.0 & \mytx{11.0}{12.0} \\
\bench{TPC-C} & 3297.3 & 763.0 & \mytx{0.9}{11.9} \\
\bench{Wikipedia} & 1067.7 & 55.1 & \mytx{8.8}{9.9} \\
\end{tabular}

% \chujun{Not sure about these column names: Default workload vs Large workload?}
% \mike{I think the large workload data should be moved to the supplementary material, similar to the other results.}

% \caption{Small workload}
% \label{subtab:bench-small}
% \end{subtable}

% \begin{subtable}[t]{\textwidth}
% \centering
% \begin{tabular}{l|rr|rr|r}
%             & \mc{2}{c|}{\bf Key--value accesses} & \mc{2}{c|}{\bf Committed transactions} & \\
% \bf Program & Reads & Writes & Total & (Read-only) & \bf Sessions \\
%   \hline
% \bench{Smallbank} & 1271.3 & 30.5 & \mytx{6.6}{20.3} & 3 \\
% \bench{Voter} & 919.0 & 6.0 & \mytx{23.0}{24.0} & 3 \\
% \bench{TPC-C} & 7025.6 & 1502.4 & \mytx{1.7}{23.8} & 3 \\
% \bench{Wikipedia} & 2677.1 & 111.1 & \mytx{20.6}{22.8} & 3 \\
% \end{tabular}
% \caption{Large workload}
% \label{subtab:bench-large}
% \end{subtable}

==> tables.tex <==
\section{Scalability Results}
\label{sec:scalability-results}

This section shows results for two workloads: the \emph{default workload} of four transactions per session from the main paper and a \emph{large workload} of eight transactions per session.

Table~\ref{tab:benchmarks_full} shows quantitative characteristics of the evaluated benchmarks for both workloads.

Tables~\ref{tab:results_full_causal} and \ref{tab:results_full_rc} show \isopredict's effectiveness and performance on both workloads under \causal and \rc, respectively.

Tables~\ref{tab:comparison_monkeydb_full:cc} and \ref{tab:comparison_monkeydb_full:rc} compare MonkeyDB and \isopredict's effectiveness at predicting \unserializable executions on both workloads.

\FloatBarrier

\begin{table*}[t]
\small
\input{results/benchmarks_full}

\caption{\label{tab:benchmarks_full} Average number of events and committed transactions across 10 trials of each OLTP-Bench program. Each execution runs 3 sessions, each of which attempts 4 transactions (default workload) or 8 transactions (large workload).}
\end{table*}

\begin{table*}
\footnotesize
\begin{subtable}[t]{\textwidth}
\centering
\input{results/oltp_cc}
\input{results/valid_cc}
\newcommand\unkOrTO{Unk}
\input{summary}
\caption{Default workload}
\end{subtable}

\begin{subtable}[t]{\textwidth}
\centering
\input{results/oltp_cc_8}
\input{results/valid_cc_8}
\newcommand\unkOrTO{T/O}
\input{summary}
% \mike{I think it doesn't make sense to use a timeout. Rather, run trials of each experiment one after the other, and see what happens. (Run trials of other experiments in parallel.) If the time taken is super long, we can report fewer trials.}
% \chujun{Comparing with the 2-hour timeout experiments, the 24-hour timeout experiments has 1 less timeout in Smallbank/Full and 5 less timeouts in TPCC/full.}
% \mike{Is that for \causal only, or \causal + \rc?}
\caption{Large workload}
\end{subtable}

\caption{\Isopredict effectiveness and performance \textbf{under \causal}.
``T/O'' means the solver did not finish within 24 hours.
``Unk'' means the solver returned ``unknown'' without reaching the timeout.}
% *\,For one trial of \bench{Wikipedia} using the \configFull strategy, the SMT solver returned ``unknown'' before reaching the timeout.}
\label{tab:results_full_causal}
\end{table*}

\begin{table*}
\footnotesize
\begin{subtable}[t]{\textwidth}
\centering
\input{results/oltp_rc}
\input{results/valid_rc}
\newcommand\unkOrTO{Unk}
\input{summary}
\caption{Default workload}
\end{subtable}

\begin{subtable}[t]{\textwidth}
\centering
\input{results/oltp_rc_8}
\input{results/valid_rc_8}
\newcommand\unkOrTO{T/O}
\input{summary}
\caption{Large workload}
\end{subtable}
\caption{\Isopredict effectiveness and performance \textbf{under \rc}.
``T/O'' means the solver did not finish within 24 hours (which did not occur in this table's results).
``Unk'' means the solver returned ``unknown'' without reaching the timeout.}
% *\,For two trials of \bench{Wikipedia} using the \configFull strategy, the SMT solver returned ``unknown'' before reaching the timeout.}
\label{tab:results_full_rc}
\end{table*}

\begin{table*}[t]
\newcommand\mynum[1]{\ifthenelse{\equal{#1}{0}}{0\%}{#1{}0\%}}
% \newcommand\mynum[1]{#1{}0\%}
% \newcommand\mynum[1]{#1/10}
\small
\begin{subtable}[h]{0.47\textwidth}
\centering
\input{results/oltp_cc}
\input{results/comparison}
\caption{Default workload}
\end{subtable}%
\hfill
\begin{subtable}[h]{0.47\textwidth}
\centering
\input{results/oltp_cc_8}
\input{results/comparison_8}
\caption{Large workload}
\end{subtable}
\caption{\label{tab:comparison_monkeydb_full:cc}Comparison between MonkeyDB~\cite{monkeydb} and \isopredict (\configRelaxed strategy) \textbf{under \causal}. Each number is the percentage of runs in which a benchmark assertion fails (\textnormal{\em Fail}) or the history is unserializable (\textnormal{\em Unser}).}


%\end{table*}
\bigskip
%\begin{table*}

% \setcounter{subtable}{0}

\begin{subtable}[h]{0.5\textwidth}
\centering
\input{results/oltp_rc}
\input{results/comparison_rc}
\caption{Default workload}
\end{subtable}%
\hfill
\begin{subtable}[h]{0.4\textwidth}
\centering
\input{results/oltp_rc_8}
\input{results/comparison_rc_8}
\caption{Large workload}
\end{subtable}
\caption{\label{tab:comparison_monkeydb_full:rc}Comparison between MonkeyDB~\cite{monkeydb}, \isopredict (\configExpress strategy), and regular execution using MySQL \textbf{under \rc}. Each number is the percentage of runs in which a benchmark assertion fails (\textnormal{\em Fail}) or the history is unserializable (\textnormal{\em Unser}).}

\end{table*}
